Cartesian Gray-Monoidal Double Categories

In this paper we present cartesian structure for symmetric Gray-monoidal double categories. To do this we first introduce locally cubical Gray categories, which are three-dimensional categorical structures analogous to classical, locally globular, Gray categories. The motivating example comprises double categories themselves, together with their functors, transformations, and modifications. A one-object locally cubical Gray category is a Gray-monoidal double category. Braiding, syllepsis, and symmetry for these is introduced in a manner analogous to that for 2-categories. Adding cartesian structure requires the introduction of doubly-lax functors of double categories to manage the order of copies. The resulting theory is algebraically rather complex, largely due to the bureaucracy of linearizing higher-dimensional boundary constraints. Fortunately, it has a relatively simple and compelling representation in the graphical calculus of surface diagrams, which we present.

==> setup/mathstyle-old.tex <==
% math settings:
\usepackage{amssymb}
\usepackage{amsmath}
	\numberwithin{equation}{section}
\usepackage{mathtools}
\usepackage{stackengine} % for combining characters
\usepackage{proof}
	\inferLineSkip=3pt % add a bit more space between lines to improve alignment (default 2pt)
	\inferLabelSkip=8pt % add a bit more space between line and label (default 5pt)
	\def\inferTabSkip{\qquad} % add a bit more space between premises (default quad)

\ifpdftex
	\usepackage{latexsym} % better \Diamond
	\usepackage{lmodern} % latin modern math(?) fonts
	\usepackage{frenchmath} % upright uppercase letters
	\usepackage{upgreek} % upright greek letters
	\usepackage{mathabx} % extensible hats and checks
	\usepackage{mathbbol} % for bbb numerals, etc. (or package bbold ?)
\else
	\usepackage{unicode-math} % should come after other math packages
	\unimathsetup
	{
		math-style = french , % italic latin lower; upright latin upper and all greek
		partial = upright ,
		nabla = upright
	}
	\setmathfont{Latin Modern Math} % must do this *after* setting the style with \unimathsetup
\fi


% fixes for unicode character support in pdftex
% and missing/bad font glyphs in xelatex
\ifpdftex
	\usepackage{newunicodechar} % declare unicode character to macro mappings for PDFLaTeX
	\newunicodechar{′}{{^{\prime}}}
	\newunicodechar{−}{-}
	\newunicodechar{×}{\times}
	\newunicodechar{∧}{\wedge}
	\newunicodechar{∨}{\vee}
	\newunicodechar{⊕}{\oplus}
	\newunicodechar{⊖}{\ominus}
	\newunicodechar{⊗}{\otimes}
	\newunicodechar{⊙}{\odot}
	\newunicodechar{⊛}{\oasterisk}
	\newunicodechar{⋅}{\cdot}
	\newunicodechar{∘}{\circ}
	\newunicodechar{∙}{\bullet}
	\newunicodechar{°}{{}^\circ}
	\newunicodechar{⋯}{\cdots}
	\newunicodechar{…}{\ldots}
	\newunicodechar{⋆}{\star}
	\newunicodechar{∞}{\infty}
	\newunicodechar{→}{\rightarrow}
	\newunicodechar{←}{\leftarrow}
	\newunicodechar{⇸}{\stackinset{c}{-0.125ex}{c}{0.25ex}{$\shortmid$}{$\rightarrow$}}%{\nrightarrow}
	\newunicodechar{⇷}{\stackinset{c}{0.125ex}{c}{0.25ex}{$\shortmid$}{$\leftarrow$}}%{\nleftarrow}
	\newunicodechar{⤍}{\dashrightarrow}
	\newunicodechar{⤌}{\dashleftarrow}
	\newunicodechar{⇒}{\Rightarrow}
	\newunicodechar{⇐}{\Leftarrow}
	\newunicodechar{↓}{\downarrow}
	\newunicodechar{↑}{\uparrow}
	\newunicodechar{⇑}{\Uparrow}
	\newunicodechar{⇓}{\Downarrow}
	\newunicodechar{↔}{\leftrightarrow}
	\newunicodechar{↦}{\mapsto}
	\newunicodechar{◇}{\Diamond}
	\newunicodechar{□}{\square}
	\newunicodechar{⟨}{\langle}
	\newunicodechar{⟩}{\rangle}
	\newunicodechar{⌜}{\ulcorner}
	\newunicodechar{⌝}{\urcorner}
	\newunicodechar{⌞}{\llcorner}
	\newunicodechar{⌟}{\lrcorner}
	\newunicodechar{∫}{\int}
	\newunicodechar{∏}{\prod}
	\newunicodechar{∐}{\coprod}
	\newunicodechar{∑}{\sum}
	\newunicodechar{≅}{\cong}
	\newunicodechar{≃}{\simeq}
	\newunicodechar{∼}{\sim}
	\newunicodechar{≔}{\coloneqq}
	\newunicodechar{≕}{\eqqcolon}
	\newunicodechar{∈}{\in}
	\newunicodechar{∋}{\ni}
	\newunicodechar{∀}{\forall}
	\newunicodechar{∃}{\exists}
	\newunicodechar{⊤}{\top}
	\newunicodechar{⊥}{\bot}
	\newunicodechar{⊢}{\vdash}
	\newunicodechar{⊣}{\dashv}
	\newunicodechar{∆}{\Delta} % should be \increment, but only in stix font
	\newunicodechar{∇}{\nabla}
	\newunicodechar{∂}{\partial}
	\newunicodechar{∞}{\infty}
	\newunicodechar{α}{\alpha}
	\newunicodechar{β}{\beta}
	\newunicodechar{γ}{\gamma}
	\newunicodechar{δ}{\delta}
	\newunicodechar{ε}{\varepsilon}
	\newunicodechar{η}{\eta}
	\newunicodechar{κ}{\kappa}
	\newunicodechar{λ}{\lambda}
	\newunicodechar{ρ}{\rho}
	\newunicodechar{μ}{\mu}
	\newunicodechar{ν}{\nu}
	\newunicodechar{π}{\pi}
	\newunicodechar{φ}{\varphi}
	\newunicodechar{ψ}{\psi}
	\newunicodechar{θ}{\theta}
	\newunicodechar{σ}{\sigma}
	\newunicodechar{τ}{\tau}
	\newunicodechar{χ}{\chi}
	\newunicodechar{ξ}{\xi}
	\newunicodechar{υ}{\upsilon}
	\newunicodechar{ζ}{\zeta}
	\newunicodechar{ω}{\omega}
	\newunicodechar{Γ}{\Gamma}
	\newunicodechar{Δ}{\Delta}
	\newunicodechar{Λ}{\Lambda}
	\newunicodechar{Φ}{\Phi}
	\newunicodechar{Ψ}{\Psi}
	\newunicodechar{Ω}{\Omega}
\else
	% fonts for characters not in default math font
	\setmathfont[range = bb]{STIX Two Math} % blackboard bold
	\setmathfont[range = {"02190,"02192}]{STIX Two Math} % ← , →
	\setmathfont[range = {"021F7,"021F8}]{STIX Two Math} % ⇷ , ⇸
	\setmathfont[range = {"0290C,"0290D}]{STIX Two Math} % ⤌ , ⤍
	\setmathfont[range = {"0219C,"0219D}]{STIX Two Math} % ↜ , ↝
	\setmathfont[range = {"02126,"02127}]{Latin Modern Math} % Ω , ℧
	\setmathfont[range = {"029C4,"029C5}]{STIX Two Math} % ⧄ , ⧅
	\setmathfont[range = "025C7]{STIX Two Math} % ◇
	\setmathfont[range = {"0250C,"02510}]{Helvetica} % ┌ , ┐
	\setmathfont[range = {"02514,"02518}]{Helvetica} % └ , ┘
\fi

